Open books and exact symplectic cobordisms

Given two open books with equal pages we show the existence of an exact symplectic cobordism whose negative end equals the disjoint union of the contact manifolds associated to the given open books, and whose positive end induces the contact manifold associated to the open book with the same page and concatenated monodromy. Using similar methods we show the existence of strong fillings for contact manifolds associated with doubled open books, a certain class of fiber bundles over the circle obtained by performing the binding sum of two open books with equal pages and inverse monodromies. From this we conclude, following an outline by Wendl, that the complement of the binding of an open book cannot contain any local filling obstruction. Given a contact $3$-manifold, according to Eliashberg there is a symplectic cobordism to a fibration over the circle with symplectic fibers. We extend this result to higher dimensions recovering a recent result by D\"orner--Geiges--Zehmisch. Our cobordisms can also be thought of as the result of the attachment of a generalized symplectic $1$-handle.

==> bib.ltb.tex <==
\bib{Ale-SystemsOfKnottedCurves}{article}{
   author={Alexander, J.~W.},
   title={A lemma on systems of knotted curves},
 %  language={English, with French summary},
   journal={Proc. Nat. Acad. Sci. U.S.A.},
   volume={9},
   date={1923}
%   number={1-2},
   pages={93--95}
%   issn={0373-0956},
%   review={\MR{1162559 (93k:57029)}},
}

\bib{2012arXiv1204.3145}{article}{
	author = {Avdek, R.}
  title = {Liouville hypersurfaces and connect sum cobordisms},
 journal = {ArXiv e-prints},
%	archivePrefix = {arXiv},
   eprint = {arXiv:1204.3145}
% keywords = {Mathematics - Symplectic Geometry, Mathematics - Geometric Topology, 57R17, 53D10},
     year = {2012}
%    month = {may},
%   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1005.1978B},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



\bib{2010arXiv1005.1978B}{article}{
	author = {Baker, K.~L.}
	author = {Etnyre, J.~B.}
	author = {Van Horn-Morris, J.},
    title = {Cabling, contact structures and mapping class monoids},
 journal = {Journal of Differential Geometry},
   volume={90},
   date={2012},
   pages={1--80}
}

% \bib{2009arXiv0909.3465E}{article}{
%    author = {Baker, K.~L.},
%    author = {Etnyre, J.~B.},
%  		author={{Van Horn-Morris}, J.},
%     title = {Cabling, contact structures and mapping class monoids},
%          year = {2009},
%        eprint = {arXiv:arXiv:0909.3465v1}
%  journal = {ArXiv e-prints}
% }

% \bib{2009arXiv0909.3465E}{article}{
%    author = {Etnyre, J.~B.},
%    author = {Baker, K.~L.},
%  		author={{Van Horn-Morris}, J.},
%     title = {Cabling, contact structures and mapping class monoids},
%          year = {2009},
%        eprint = {arXiv:arXiv:0909.3465v1}
%  journal = {ArXiv e-prints}
% }

\bib{arXiv1005.2169v1}{article}{
   author={Baldwin, J.~A.},
   title={Contact monoids and Stein cobordisms},
 journal = {ArXiv e-prints},
   eprint = {arXiv:1005.2169v1}
   date={2010}
}


\bib{MR2923174}{article}{
   author={Baldwin, J.~A.},
   title={Contact monoids and Stein cobordisms},
   journal={Math. Res. Lett.},
   volume={19},
   date={2012},
   %number={1},
   pages={31--40}
   %issn={1073-2780},
   %review={\MR{2923174}},
   %doi={10.4310/MRL.2012.v19.n1.a4},
}
	

%[DGZ, Open books and the Weinstein conjecture, in preparation]


\bib{MR2385640}{article}{
   author={Baldwin, J.~A.},
   title={Comultiplicativity of the Ozsv\'ath-Szab\'o contact invariant},
   journal={Math. Res. Lett.},
   volume={15},
   date={2008},
%   number={2},
   pages={273--287}
%   issn={1073-2780}
%   review={\MR{2385640 (2009c:57043)}},
}



\bib{MR1447038}{article}{
   author={Colin, V.},
   title={Chirurgies d'indice un et isotopies de sph\`eres dans les
   vari\'et\'es de contact tendues},
 %  language={French, with English and French summaries},
   journal={C. R. Acad. Sci. Paris S\'er. I Math.},
   volume={324},
   date={1997},
%   number={6},
   pages={659--663}
%   issn={0764-4442},
%   review={\MR{1447038 (98e:57036)}},
%   doi={10.1016/S0764-4442(97)86985-6},
}

\bib{MaxThesis}{article}{
   author={D\"orner, M.},
   title = {The Space of Contact Forms Adapted to an Open Book},
   journal={Dissertation, University of Cologne, Germany},
  %eprint={arXiv:1210.7947},
  date={2014}
} 

\bib{DGZ}{article}{
   author={D{\"o}rner, M.},
   author={Geiges, H.},
   author={Zehmisch, K.},
   title={Open books and the Weinstein conjecture},
   journal={Q. J. Math.},
   volume={65},
   date={2014},
   %number={3},
   pages={869--885}
   %issn={0033-5606},
   %review={\MR{3261972}},
   %doi={10.1093/qmath/hat055},
}


\bib{El20years}{article}{
   author={Eliashberg, Y.},
   title={Contact $3$-manifolds twenty years since J. Martinet's work},
 %  language={English, with French summary},
   journal={Ann. Inst. Fourier (Grenoble)},
   volume={42},
   date={1992}
%   number={1-2},
   pages={165--192}
%   issn={0373-0956},
%   review={\MR{1162559 (93k:57029)}},
}

\bib{MR1162559}{article}{
   author={Eliashberg, Y.},
   title={Contact $3$-manifolds twenty years since J. Martinet's work},
   language={English, with French summary},
   journal={Ann. Inst. Fourier (Grenoble)},
   volume={42},
   date={1992},
%   number={1-2},
   pages={165--192}
%   issn={0373-0956},
%   review={\MR{1162559 (93k:57029)}},
}


\bib{MR1022310}{article}{
   author={Eliashberg, Y.},
   title={Classification of overtwisted contact structures on $3$-manifolds},
   journal={Invent. Math.},
   volume={98},
   date={1989},
%   number={3},
   pages={623--637}
%   issn={0020-9910},
%   review={\MR{1022310 (90k:53064)}},
%   doi={10.1007/BF01393840},
}

\bib{MR2023279}{article}{
   author={Eliashberg, Y.},
   title={A few remarks about symplectic filling},
   journal={Geom. Topol.},
   volume={8},
   date={2004},
   pages={277--293}
%   issn={1465-3060},
%   review={\MR{2023279 (2005a:57022b)}},
%   doi={10.2140/gt.2004.8.277},
}

\bib{MR2496415}{article}{
   author={Eliashberg, Yakov},
   author={Fraser, Maia},
   title={Topologically trivial Legendrian knots},
   journal={J. Symplectic Geom.},
   volume={7},
   date={2009},
%   number={2},
   pages={77--127},
   issn={1527-5256},
   review={\MR{2496415 (2010d:57024)}},
}


\bib{EliFraTTLK}{article}{
   author={Eliashberg, Y.},
   author={Fraser, M.},
   title={Topologically trivial Legendrian knots},
   journal={J. Symplectic Geom.},
   volume={7},
   date={2009},
%   number={2},
   pages={77--127}
%   issn={1527-5256},
%   review={\MR{2496415 (2010d:57024)}},
}

\bib{MR1044658}{article}{
   author={Eliashberg, Y.},
   title={Topological characterization of Stein manifolds of dimension
   $>2$},
   journal={Internat. J. Math.},
   volume={1},
   date={1990},
%   number={1},
   pages={29--46}
%   issn={0129-167X},
%   review={\MR{1044658 (91k:32012)}},
%   doi={10.1142/S0129167X90000034},
}

\bib{MR1128541}{article}{
   author={Eliashberg, Yakov},
   author={Gromov, Mikhael},
   title={Convex symplectic manifolds},
   conference={
      title={Several complex variables and complex geometry, Part 2 (Santa
      Cruz, CA, 1989)},
   },
   book={
      series={Proc. Sympos. Pure Math.},
      volume={52},
      publisher={Amer. Math. Soc.},
      place={Providence, RI},
   },
   date={1991},
   pages={135--162},
   review={\MR{1128541 (93f:58073)}},
}


\bib{eliGro-convex_symplectic_manifolds}{article}{
   author={Eliashberg, Y.},
   author={Gromov, M.},
   title={Convex symplectic manifolds},
   conference={
      title={Several complex variables and complex geometry, Part 2 (Santa
      Cruz, CA, 1989)},
   },
   book={
      series={Proc. Sympos. Pure Math.},
      volume={52},
      publisher={Amer. Math. Soc.},
      place={Providence, RI},
   },
   date={1991},
   pages={135--162}
%   review={\MR{1128541 (93f:58073)}},
}

\bib{MR2249250}{article}{
   author = {Etnyre, J.~B.},
   title={Lectures on open book decompositions and contact structures},
   conference={
      title={Floer homology, gauge theory, and low-dimensional topology},
   },
   book={
      series={Clay Math. Proc.},
      volume={5},
      publisher={Amer. Math. Soc.},
      place={Providence, RI},
   },
   date={2006},
   pages={103--141}
%   review={\MR{2249250 (2007g:57042)}},
}

\bib{MR2407103}{article}{
   author = {Etnyre, J.~B.},
   title={On contact surgery},
   journal={Proc. Amer. Math. Soc.},
   volume={136},
   date={2008},
%   number={9},
   pages={3355--3362}
%   issn={0002-9939},
%   review={\MR{2407103 (2010b:57036)}},
%   doi={10.1090/S0002-9939-08-09278-2},
}

\bib{2010arXiv1012.3745E}{article}{
   author = {Etnyre, J.~B.},
    title = {On knots in overtwisted contact structures},
  journal = {ArXiv e-prints},
  eprint={arXiv:1012.3745},
  date={2010}
}

\bib{etn-on_symplectic_cobordisms}{article}{
   author = {Etnyre, J.~B.},
      author = {Honda, K.},
    title = {On symplectic cobordisms}
}

\bib{MR2023278}{article}{
   author={Etnyre, John B.},
   title={On symplectic fillings},
   journal={Algebr. Geom. Topol.},
%   volume={4},
   date={2004},
   pages={73--80}
%   issn={1472-2747},
%   review={\MR{2023278 (2005a:57022a)}},
%   doi={10.2140/agt.2004.4.73},
}



\bib{etn-convex_notes}{article}{
   author = {Etnyre, J.~B.},
   title={Convex surfaces in contact geometry: Class notes},
   date={2004},
   eprint={http://people.math.gatech.edu/~etnyre/preprints/papers/surfaces.pdf}
}

\bib{MR2024641}{article}{
   author = {Etnyre, J.~B.},
   author={Ng, L.},
   title={Problems in low dimensional contact topology},
   conference={
      title={Topology and geometry of manifolds},
      address={Athens, GA},
      date={2001},
   },
   book={
      series={Proc. Sympos. Pure Math.},
      volume={71},
      publisher={Amer. Math. Soc.},
      place={Providence, RI},
   },
   date={2003},
   pages={337--357}
%   review={\MR{2024641 (2004k:57033)}},
}

\bib{2009arXiv0909.3465E}{article}{
   author = {Etnyre, J.~B.},
   author = {Vela-Vick, D.~S.},
    title = {Torsion and open book decompositions},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
   eprint = {arXiv:0909.3465},
% keywords = {Mathematics - Symplectic Geometry, Mathematics - Geometric Topology, 57M27, 57R58},
     year = {2009}
%    month = {sep},
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0909.3465E},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR2737776}{article}{
   author={Etnyre, J.~B.},
   author={Vela-Vick, D.~S.},
   title={Torsion and open book decompositions},
   journal={Int. Math. Res. Not. IMRN},
   date={2010},
   %number={22},
   pages={4385--4398}
   %issn={1073-7928},
   %review={\MR{2737776 (2011j:57035)}},
   %doi={10.1093/imrn/rnq054},
}
	




\bib{FucTab1}{article}{
   author = {Fuchs, D.},
   author = {Tabachnikov, S.},
    title = {Invariants of Legendrian and transverse knots in the standard 
contact space}
}

\bib{MR2350472}{article}{
   author = {Gay, D.~T.},
   author = {Kirby, R.},
   title={Constructing Lefschetz-type fibrations on four-manifolds},
   journal={Geom. Topol.},
   volume={11},
   date={2007},
   pages={2075--2115}
%   issn={1465-3060}
}

\bib{2009arXiv0908.3774G}{article}{
   author = {Gay, D.~T.},
   author = {Stipsicz, A.~I.},
    title = {On symplectic caps},
  journal = {ArXiv e-prints},
   eprint = {arxiv:0908.3774},
% keywords = {Mathematics - Symplectic Geometry, Mathematics - Geometric Topology},
     year = {2009}
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0908.3774G},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




\bib{MR2397738}{book}{
   author={Geiges, H.},
   title={An Introduction to Contact Topology},
   series={Cambridge Studies in Advanced Mathematics},
   volume={109},
   publisher={Cambridge University Press},
   place={Cambridge},
   date={2008},
   pages={xvi+440}
%   isbn={978-0-521-86585-2},
%   review={\MR{2397738 (2008m:57064)}},
%   doi={10.1017/CBO9780511611438},
}

\bib{2003math......3303G}{article}{
   author={Geiges, H.},
   author={Gonzalo, J.},
   title={On the topology of the space of contact structures on torus
   bundles},
   journal={Bull. London Math. Soc.},
   volume={36},
   date={2004},
%   number={5},
   pages={640--646}
%   issn={0024-6093},
%   review={\MR{2070440 (2005f:53153)}},
%   doi={10.1112/S0024609304003376},
}




%[DGZ, Open books and the Weinstein conjecture, in preparation]


\bib{MR2070440}{article}{
   author={Geiges, H.},
   author={Gonzalo, J.},
   title={On the topology of the space of contact structures on torus
   bundles},
   journal={Bull. London Math. Soc.},
   volume={36},
   date={2004},
%   number={5},
   pages={640--646}
%   issn={0024-6093},
%   review={\MR{2070440 (2005f:53153)}},
%   doi={10.1112/S0024609304003376},
}

\bib{GeiGon-15YearsOfContactSpheres}{article}{
   author={Geiges, H.},
    author= {Gonzalo, J.},
    title = {Fifteen years of contact circles and contact spheres},
  journal = {unpublished}
}

\bib{2009arXiv0903.1488D}{article}{
   author={Ding, F.},
   author={Geiges, H.},
    title = {The diffeotopy group of S\^{}1 $\backslash$times S\^{}2 via contact topology},
  journal = {ArXiv e-prints},
	date = {2009}
}

\bib{MR2455948}{article}{
   author={Ding, F.},
   author={Geiges, H.},
   title={A unique decomposition theorem for tight contact 3-manifolds},
   journal={Enseign. Math. (2)},
   volume={53},
   date={2007},
%   number={3-4},
   pages={333--345}
%   issn={0013-8584},
%   review={\MR{2455948 (2009k:57042)}},
}


\bib{2010arXiv1012.1721G}{article}{
   author={Ding, F.},
   author={Geiges, H.},
    title = {Neighbourhoods and isotopies of knots in contact $3$-manifolds},
%  eprint= {arXiv:1012.1721},
%  	date = {2010},
  	  journal={Arch. Math. (Basel)},
   volume={97},
   date={2011},
   pages={391--397}
}

\bib{MR1823497}{article}{
   author={Ding, F.},
   author={Geiges, H.},
   title={Symplectic fillability of tight contact structures on torus
   bundles},
   journal={Algebr. Geom. Topol.},
   volume={1},
   date={2001},
   pages={153--172 }
%   issn={1472-2747},
%   review={\MR{1823497 (2002b:53134)}},
%   doi={10.2140/agt.2001.1.153},
}


\bib{MR2056760}{article}{
   author={Ding, F.},
   author={Geiges, H.},
   author={Stipsicz, A.~I.},
   title={Surgery diagrams for contact $3$-manifolds},
   journal={Turkish J. Math.},
   volume={28},
   date={2004},
%   number={1},
   pages={41--74}
%   issn={1300-0098},
%   review={\MR{2056760 (2005c:57028)}},
}


\bib{MR2225643}{article}{
   author={Ghiggini, P.},
   title={Linear Legendrian curves in $T^3$},
   journal={Math. Proc. Cambridge Philos. Soc.},
   volume={140},
   date={2006},
%   number={3},
   pages={451--473}
%   issn={0305-0041},
%   review={\MR{2225643 (2007a:57031)}},
%   doi={10.1017/S0305004105009151},
}



\bib{MR2180909}{article}{
   author={Ghiggini, P.},
   author={Lisca, P.},
   author={Stipsicz, Andr{\'a}s I.},
   title={Classification of tight contact structures on small Seifert
   3-manifolds with $e_0\geq 0$},
   journal={Proc. Amer. Math. Soc.},
   volume={134},
   date={2006},
%   number={3},
   pages={909--916 }
%   issn={0002-9939},
%   review={\MR{2180909 (2006m:57036)}},
%   doi={10.1090/S0002-9939-05-08013-5},
}
	

\bib{MR1957051}{article}{
   author={Giroux, E.},
   title={G\'eom\'etrie de contact: de la dimension trois vers les
   dimensions sup\'erieures},
%   language={French, with French summary},
   conference={
      title={},
      address={Beijing},
      date={2002},
   },
   book={
      publisher={Higher Ed. Press},
      place={Beijing},
   },
   date={2002},
   pages={405--414}
%   review={\MR{1957051 (2004c:53144)}},
}

\bib{MR2511589}{article}{
   author={Colin, V.},
   author={Giroux, E.},
   author={Honda, K.},
   title={Finitude homotopique et isotopique des structures de contact
   tendues},
%   language={French, with French summary},
   journal={Publ. Math. Inst. Hautes \'Etudes Sci.},
%   number={109},
   date={2009},
   pages={245--293}
%   issn={0073-8301},
%   review={\MR{2511589 (2010g:53167)}},
%   doi={10.1007/s10240-009-0022-y},
}



\bib{2001math......2009G}{article}{
   author={Giroux, E.},
    title = {Sur les transformations de contact au-dessus des surfaces},
%  journal = {ArXiv Mathematics e-prints},
   eprint = {arXiv:math/0102009},
% keywords = {Geometric Topology, Symplectic Geometry, Differential Geometry, 57M50, 57R17 (primary) 53D35, 53D10 (secondary)},
     year = {2001}
%   adsurl = {http://adsabs.harvard.edu/abs/2001math......2009G},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{1999math.....11235G}{article}{
   author={Giroux, E.},
    title = {Structures de contact sur les varietes fibrees en cercles au-dessus d'une surface},
%  journal = {ArXiv Mathematics e-prints},
   eprint = {arXiv:math/9911235},
% keywords = {Mathematics - Geometric Topology, Mathematics - Differential Geometry, Mathematics - Symplectic Geometry, 57M50, 57R17 (primary) 53D35, 53D10 (secondary)},
     year = {1999}
%    month = nov,
%   adsurl = {http://adsabs.harvard.edu/abs/1999math.....11235G},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR1129802}{article}{
   author={Giroux, E.},
   title={Convexit\'e en topologie de contact},
%   language={French},
   journal={Comment. Math. Helv.},
   volume={66},
   date={1991},
%   number={4},
   pages={637--677}
%   issn={0010-2571},
%   review={\MR{1129802 (93b:57029)}},
%   doi={10.1007/BF02566670},
}

\bib{MR1779622}{article}{
   author={Giroux, E.},
   title={Structures de contact en dimension trois et bifurcations des
   feuilletages de surfaces},
%   language={French},
   journal={Invent. Math.},
   volume={141},
   date={2000},
%   number={3},
   pages={615--689}
%   issn={0020-9910},
%   review={\MR{1779622 (2001i:53147)}},
%   doi={10.1007/s002220000082},
}



\bib{MR2207791}{article}{
   author={Giroux, E.},
   author={Goodman, N.},
   title={On the stable equivalence of open books in three-manifolds},
   journal={Geom. Topol.},
%   volume={10},
   date={2006},
   pages={97--114}
%   issn={1465-3060},
%   review={\MR{2207791 (2006k:57046)}},
%   doi={10.2140/gt.2006.10.97},
}
		




\bib{MR2171807}{article}{
   author={Goodman, N.},
   title={Overtwisted open books from sobering arcs},
   journal={Algebr. Geom. Topol.},
   volume={5},
   date={2005},
   pages={1173--1195}
%   issn={1472-2747},
%   review={\MR{2171807 (2006h:57022)}},
%   doi={10.2140/agt.2005.5.1173},
}



\bib{MR0098847}{article}{
   author={Grauert, H.},
   title={On Levi's problem and the imbedding of real-analytic manifolds},
   journal={Ann. of Math. (2)},
   volume={68},
   date={1958},
   pages={460--472}
%   issn={0003-486X},
%   review={\MR{0098847 (20 \#5299)}},
}
		



\bib{MR1940409}{article}{
   author={Honda, K.},
   title={Gluing tight contact structures},
   journal={Duke Math. J.},
   volume={115},
   date={2002},
%   number={3},
   pages={435--478}
%   issn={0012-7094},
%   review={\MR{1940409 (2003i:53125)}},
%   doi={10.1215/S0012-7094-02-11532-4},
}

\bib{MR1786111}{article}{
   author={Honda, K.},
   title={On the classification of tight contact structures. I},
   journal={Geom. Topol.},
   volume={4},
   date={2000},
   pages={309--368}
%   issn={1465-3060},
%   review={\MR{1786111 (2001i:53148)}},
%   doi={10.2140/gt.2000.4.309},
}

\bib{hon-tight-classification-1}{article}{
   author={Honda, K},
   title={On the classification of tight contact structures. I},
   journal={Geom. Topol.},
   volume={4},
   date={2000},
   pages={309--368}
%   issn={1465-3060},
%   review={\MR{1786111 (2001i:53148)}},
%   doi={10.2140/gt.2000.4.309},
}

\bib{2008arXiv0807.2431H}{article}{
   author = {Honda, K.},
   author = {Kazez, W.~H.},
   author = {Matic, G.},
    title = {Contact structures, sutured Floer homology and TQFT},
  eprint = {arXiv:0807.2431},
     date = {2008}
}
\bib{2007arXiv0705.2828H}{article}{
   author = {Honda, K.},
   author = {Kazez, W.~H.},
   author = {Matic, G.},
    title = {The contact invariant in sutured Floer homology},
  eprint = {	arXiv:0705.2828},
     date = {2007}
}

\bib{MR1874319}{article}{
   author={Honda, Ko},
   author={Kazez, William H.},
   author={Mati{\'c}, Gordana},
   title={Convex decomposition theory},
   journal={Int. Math. Res. Not.},
   date={2002},
%   number={2},
   pages={55--88}
%   issn={1073-7928},
%   review={\MR{1874319 (2002k:57064)}},
%   doi={10.1155/S1073792802101140},
}


\bib{2009arXiv0910.4382J}{article}{
   author = {Juh\'{a}sz, A.},
    title = {Cobordisms of sutured manifolds},
  journal = {ArXiv e-prints},
   eprint = {arXiv:0910.4382},
  	year  = {2009}
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0910.4382J},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR2253454}{article}{
   author={Juh{\'a}sz, A.},
   title={Holomorphic discs and sutured manifolds},
   journal={Algebr. Geom. Topol.},
   volume={6},
   date={2006},
   pages={1429--1457}
%   issn={1472-2747},
%   review={\MR{2253454 (2007g:57024)}},
%   doi={10.2140/agt.2006.6.1429},
}





\bib{MR1487723}{article}{
   author={Kanda, Y.},
   title={The classification of tight contact structures on the $3$-torus},
   journal={Comm. Anal. Geom.},
   volume={5},
   date={1997},
%   number={3},
   pages={413--438}
%   issn={1019-8385},
%   review={\MR{1487723 (99c:57054)}},
}

\bib{MR1632790}{article}{
   author={Kanda, Y.},
   title={On the Thurston-Bennequin invariant of Legendrian knots and
   nonexactness of Bennequin's inequality},
   journal={Invent. Math.},
   volume={133},
   date={1998},
%   number={2},
   pages={227--242}
%   issn={0020-9910},
%   review={\MR{1632790 (99g:57030)}},
%   doi={10.1007/s002220050245},
}



\bib{MR1487723}{article}{
   author={Kanda, Y.},
   title={The classification of tight contact structures on the $3$-torus},
   journal={Comm. Anal. Geom.},
   volume={5},
   date={1997},
%   number={3},
   pages={413--438}
%   issn={1019-8385},
%   review={\MR{1487723 (99c:57054)}},
}

\bib{Klukas-Thesis}{article}{
   author={Klukas, M.},
   title={Constructions of open book decompositions and applications of convex surfaces in contact topology},
   journal={Dissertation, University of Cologne, Germany},
   %eprint = {http://www.aimath.org/~jvanhorn/dissertation-jvhm.pdf},
   date={submitted March 2012}
}

		
\bib{MassotThesis}{article}{
   author={Massot, P.},
   title={Thesis - Sur\ldots}
}

\bib{2009arXiv0912.5107M}{article}{
   author = {Massot, P.},
    title = {Infinitely many universally tight torsion free contact structures with vanishing Ozsv\'ath-Szab\'o contact invariants},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
eprint = {arXiv:0912.5107},
     year = {2009}
%    month = {dec},
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0912.5107M},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR1487640}{book}{
   author={Milnor, J.~W.},
   title={Topology from the Differentiable Viewpoint},
   series={Princeton Landmarks in Mathematics},
%   note={Based on notes by David W. Weaver;
%   Revised reprint of the 1965 original},
   publisher={Princeton University Press},
   place={Princeton, NJ},
   date={1997},
   pages={xii+64}
%   isbn={0-691-04833-9},
%   review={\MR{1487640 (98h:57051)}},
}



\bib{2009arXiv0905.0986O}{article}{
   author = {Ozbagci, B.},
   author = {Pamuk, M.},
    title = {Full Lutz twist along the binding of an open book},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
   eprint = {arXiv:0905.0986},
% keywords = {Mathematics - Geometric Topology, 57R17},
     year = {2009}
%    month = {may},
%   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0905.0986O},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\bib{MR1414898}{book}{
   author={Prasolov, V.~V.},
   author={Sossinsky, A.~B.},
   title={Knots, Links, Braids and $3$-Manifolds},
   series={Translations of Mathematical Monographs},
   volume={154},
%   note={An introduction to the new invariants in low-dimensional topology;
%   Translated from the Russian manuscript by Sossinsky [Sosinski\u\i]},
   publisher={American Mathematical Society},
   place={Providence, RI},
   date={1997},
   pages={viii+239}
%   isbn={0-8218-0588-6},
%   review={\MR{1414898 (98i:57018)}},
}



\bib{vanHornMorris-Thesis}{article}{
   author={{Van Horn-Morris}, J.},
   title={Constructions of open book decompositions},
   journal={Dissertation, University of Texas at Austin},
   eprint = {http://www.aimath.org/~jvanhorn/dissertation-jvhm.pdf},
   date={2007}
}

\bib{MR0375366}{article}{
   author={Thurston, W.~P.},
   author={Winkelnkemper, H.~E.},
   title={On the existence of contact forms},
   journal={Proc. Amer. Math. Soc.},
   volume={52},
   date={1975},
   pages={345--347}
%   issn={0002-9939},
%   review={\MR{0375366 (51 \#11561)}},
}

\bib{MR1114405}{article}{
   author={Weinstein, A.},
   title={Contact surgery and symplectic handlebodies},
   journal={Hokkaido Math. J.},
   volume={20},
   date={1991},
%   number={2},
   pages={241--251}
%   issn={0385-4035},
%   review={\MR{1114405 (92g:53028)}},
}

\bib{2010arXiv1009.2746W}{article}{
   author = {Wendl, C.},
    title = {A hierarchy of local symplectic filling obstructions for contact $3$-manifolds},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
   eprint = {arXiv:1009.2746},
   date = {2010}
% yearsurl = {ttp://adsabs.harvard.edu/abs/2010arXiv1009.2746W}
}

\bib{MR3102479}{article}{
   author={Wendl, C.},
   title={A hierarchy of local symplectic filling obstructions for contact
   3-manifolds},
   journal={Duke Math. J.},
   volume={162},
   date={2013},
   %number={12},
   pages={2197--2283}
   %issn={0012-7094},
   %review={\MR{3102479}},
   %doi={10.1215/00127094-2348333},
}

\bib{2010arXiv1008.2456v2}{article}{
   author = {Wendl, C.},
    title = {Non-exact symplectic cobordisms between contact
3-manifolds},
  journal = {ArXiv e-prints},
%archivePrefix = {arXiv},
   eprint = {	arXiv:1008.2456v2},
   date = {2010}
% yearsurl = {ttp://adsabs.harvard.edu/abs/2010arXiv1009.2746W}
}

\bib{MR3128981}{article}{
   author={Wendl, C.},
   title={Non-exact symplectic cobordisms between contact 3-manifolds},
   journal={J. Differential Geom.},
   volume={95},
   date={2013},
   %number={1},
   pages={121--182}
   %issn={0022-040X},
   %review={\MR{3128981}},
}



\bib{2010arXiv1010.3496Z}{article}{
   author = {Zarev, R.},
    title = {Joining and gluing sutured Floer homology},
  journal = {ArXiv e-prints},
 keywords = {Mathematics - Geometric Topology, Mathematics - Symplectic Geometry, 57R58, 57M27},
     date = {2010}
}


